On the Equivalence Between Abstract Dialectical Frameworks and Logic Programs

Abstract Dialectical Frameworks (ADFs) are argumentation frameworks where each node is associated with an acceptance condition. This allows us to model different types of dependencies as supports and attacks. Previous studies provided a translation from Normal Logic Programs (NLPs) to ADFs and proved the stable models semantics for a normal logic program has an equivalent semantics to that of the corresponding ADF. However, these studies failed in identifying a semantics for ADFs equivalent to a three-valued semantics (as partial stable models and well-founded models) for NLPs. In this work, we focus on a fragment of ADFs, called Attacking Dialectical Frameworks (ADF$^+$s), and provide a translation from NLPs to ADF$^+$s robust enough to guarantee the equivalence between partial stable models, well-founded models, regular models, stable models semantics for NLPs and respectively complete models, grounded models, preferred models, stable models for ADFs. In addition, we define a new semantics for ADF$^+$s, called L-stable, and show it is equivalent to the L-stable semantics for NLPs. This paper is under consideration for acceptance in TPLP.

==> dialectical.tex <==
\section{ Abstract Dialectical Frameworks}\label{s:dialectical}

Abstract Dialectical Frameworks have been designed in \cite{brewka2010abstract} to treat arguments (called statements there) as abstract and atomic entities. It can be seen as a directed graph whose nodes represent statements which can be accepted or not. In addition, the links between nodes represent dependencies: the status of a node $s$ only depends on the status of its parents (denoted $\pr(s)$), that is, the nodes with a direct link to $s$. 

In this paper, we will propose a slight change in this approach: instead of resorting to subsets of $\pr(s)$ to assess the status of $s$, we will make this dependency between statements more explicit by resorting to subsets of $\lit(s)$:
\[ \lit(s) = \pr(s) \cup \set{\neg s' \mid s' \in \pr(s)} \]

A set $M \subseteq \lit(s)$ is consistent iff there is no statement $s \in \pr(s)$ such that $\set{s, \neg s} \subseteq M$. We denote by $\mathfrak C_s = \set{M \subseteq \lit(s) \mid M \textit{ is consistent}}$ the set of all consistent subsets of $\lit(s)$. We will refer to $a \in S$ as a positive (resp. negative) statement in $M$ if $a \in M$ (resp. $\neg a \in M$). Now we can alter accordingly the original definition of Abstract Dialectical Frameworks \cite{brewka2010abstract} as follows:

\begin{mdef}[Abstract Dialectical Frameworks]\label{d:adf}
An abstract dialectical framework is a tuple $D = (S, L, C)$ where

\begin{itemize}
    \item $S$ is a set of statements (positions, nodes),
    \item $L \subseteq S \times S$ is a set of links,
    \item $C = \set{C_s \mid s \in S}$ is a set of total functions $C_s : \mathfrak C_s \to \set{\tr, \fa}$, one for each statement $s$, such that for any $M \in \mathfrak C_s$, if $C_s(M) = \tr$, then $C_s(M') = \tr$\@  for any $M' \supseteq M$. $C_s$ is called acceptance condition of $s$.
\end{itemize}
\end{mdef}

The set $C_s$ for a statement $s$ is intended to determine the acceptance status of $s$, which as before only depends on the status of its parent nodes $\pr(s)$. The novelty is that now for each node $s \in S$, its acceptance condition $C_s$ specifies \emph{explicitly} the exact conditions under which $s$ is accepted, giving room to a (partial) three-valued setting. Intuitively, 

\begin{itemize}
    \item $s$ will be accepted if there exists $M \subseteq \mathfrak C_s$ such that $C_s(M) = \tr$ and every positive statement in $M$ is accepted and every negative statement in $M$ is rejected.
    \item $s$ will be rejected if for every $M \subseteq \mathfrak C_s$ such that $C_s(M) = \tr$, there exists either a rejected positive statement in $M$ or an accepted negative statement in $M$.
    \item $s$ will be undefined otherwise. 
\end{itemize}

The acceptance conditions in $C$ of an $\adf (S, L, C)$ can also be represented in two alternative ways:

\begin{itemize}
    \item Any function $C_s \in C$ can be represented by the set of subsets of $\mathfrak C_s$ leading to acceptance, i.e.,  $C^\tr = \set{C^\tr_s \mid s \in S}$, where $C^\tr_s = \{M \in \mathfrak C_s \mid C_s(M) = \tr \}$. We will indicate this alternative by denoting an $\adf$ as $(S, L, C^\tr)$.
    \item Any function $C_s \in C$ can also be represented as a propositional formula $\varphi_s$ over the vocabulary $\mathfrak C_s$ as follows:
\[ \varphi_s \equiv \bigvee_{\set{a_1, \ldots, a_m, \neg b_1, \ldots, \neg b_n} \in C^\tr_s} a_1 \wedge \cdots \wedge a_m \wedge \neg b_1 \wedge \cdots \wedge \neg b_n \]
If $m = n = 0$, the corresponding $a_1 \wedge \cdots \wedge a_m \wedge \neg b_1 \wedge \cdots \wedge \neg b_n \equiv \top$, where $\top$ is a constant always evaluated as $\tr$. If there is no $M \in \mathfrak C_s$ such that $C_s(M) = \tr$, then $\phi_s \equiv \bot$, where $\bot$ is a constant always evaluated as $\fa$. By $C^\varphi$ we mean the set $\set{\varphi_s \mid s \in S}$. We will indicate this alternative by denoting an $\adf$ as $(S, L, C^\varphi)$.
\end{itemize}

When referring to an $\adf$ as $(S, L, C^\varphi)$, we will assume the acceptance formulas specify implicitly the parents a node depends on. Then the set $L$ of links between statements can be ignored, and the $\adf$ can be represented as $(S, C^\varphi)$, where $L$ is recovered by $(a,b) \in L$ iff $a$ appears in $\phi_b$.

In order to define different semantics for $\adf $s over statements $s$, we will resort to the notion of admissible labellings:

\begin{mdef}[Admissible Labellings]\label{d:admissible}
Let $D = (S, C^\varphi)$ be an $\adf$. A three-valued labelling is a mapping $v : S \to \set{\tr, \fa, \un}$ that assigns the values ($\tr$), ($\fa$), or ($\un$) to each statement $s$. Labellings will be extended to assign values to formulas over statements according to Kleene's strong three-valued logic \cite{kleene1952introduction}: negation switches $\tr$ and $\fa$, and leaves $\un$ unchanged; a conjunction is $\tr$ if both conjuncts are $\tr$, it is $\fa$ if some conjunct is $\fa$ and it is $\un$ otherwise; disjunction is dual. Sometimes, when convenient, we will refer to a labelling $v$ over $S$ as a set $V = \set{s \mid s \in S \textit{ and } v(s) = \tr} \cup \set{\neg s \mid s \in S \textit{ and } v(s) = \fa}$. Obviously, if neither $s \in S$ nor $\neg s \in S$, then $v(s) = \un$.

A three-valued labelling $v$ is an admissible labelling of $D$ iff for all $s \in S$, if $v(s) \neq \un$, then $v(s) = v(\varphi_s)$.
\end{mdef}

Admissible labellings can also be characterized as follows:

\begin{restatable}{prop}{admissible}\label{p:admissible}
Let $D = (S, L, C^\tr)$ be an $\adf$, and for any three-valued labelling $v : S \to \set{\tr, \fa, \un}$, let $M_v = \set{s \mid v(s) = \tr} \cup \set{\neg s \mid v(s) = \fa}$. Then $v$ is an admissible labelling of $D$ iff for any $s \in S$
\begin{itemize}
    \item $s \in M_v$ iff $M_v \cap \lit(s) \in C^\tr_s$; 
    \item $\neg s \in M_v$ iff for all $M' \in C^\tr_s$, we have $M' \not\subseteq M_v$.
\end{itemize}

\end{restatable}

Besides admissible labellings, complete labellings are a crucial notion employed in the definitions of the semantics for an $\adf$:

\begin{mdef}[Complete labellings]\label{d:complete}
Let $D = (S, L, C^\tr)$ be an $\adf$. A three-valued labelling $v$ over $S$ is complete iff for all $s \in S$, $v(s) = v(\varphi_s)$.
\end{mdef}


The truth-values $\tr$, $\fa$ and $\un$ are partially ordered by $\leq_i$ according to their information content: $\un \leq_i \fa$ and $\un \leq_i \tr$, whereas $\tr$ and $\fa$ are incomparable. The intended meaning of $\leq_i$ is both $\tr$ and $\fa$ are more informative than $\un$. The pair $(\set{\tr, \fa, \un}, \leq_i)$ is a complete meet-semilattice, i.e., every non-empty subset of $V = \set{\tr, \fa, \un}$ has a greatest lower-bound (meet), and every directed subset $B \subseteq V$ (any two elements of $B$ have an upper bound in $B$), has a least upper bound.

The information ordering $\leq_i$ is extended to labellings $v_1, v_2$ over $S$: $v_1 \leq_i v_2$ iff $v_1(s) \leq_i v_2(s)$ for all $s \in S$. Let $\mathfrak V_S$ be the set of all three-valued labellings over $S$. The pair $(\mathfrak V_s, \leq_i)$ is a complete meet-semilattice, where the consensus meet operation $\sqcap$ of this semilattice is given by $v_1 \sqcap v_2 = v_1(s) \cap v_2(s)$ for all $s \in S$. The valuation $v(s) = \un$ for every $s \in S$ is the least element of this semilattice.

The semantics for an $\adf$ will be based on the operator $\Gamma_D$ over three-valued labellings:

\begin{mdef}[$\Gamma_D$ Operator]\label{d:gamma} Let $D = (S, L, C^\varphi)$ be an $\adf$, and $v$ a three-valued labelling over $S$. We define $\Gamma_D(v) = v'$, where $v'(s) = v(\varphi_s)$ for any $s \in S$.
\end{mdef}

We say $v$ is a fixpoint of $\Gamma_D$ if $\Gamma_D(v) = v$; it is a pre-fixpoint of $\Gamma_D$ if $\Gamma_D(v) \leq_i v$; it is a post-fixpoint of $\Gamma_D$ if $v \leq_i \Gamma_D(v)$. The following result suffices to guarantee each $\adf$ has a unique least fixpoint/pre-fixpoint: 

\begin{restatable}{prop}{monotonic}\label{p:monotonic}
For any $\adf$ $D = (S, L, C^\varphi)$, the operator $\Gamma_D$ is $\leq_i$-monotone.
\end{restatable}

 Hence, due to the fundamental result by Tarski and Knaster \cite{tarski1955lattice}, the $\leq_i$-least pre-fixpoint and also the $\leq_i$-least fixpoint are unique (indeed, they coincide with each other) and guaranteed to exist. Besides, the set of fixpoints of $\Gamma_D$ forms a complete meet-semilattice with respect to  $\leq_i$:
 
 \begin{restatable}{theo}{semilattice}\label{t:semilattice}
 Let $D$ be an $\adf$. The complete labellings of $D$ form a complete meet-semilattice with respect to $\leq_i$.
 \end{restatable}

The next results show how $\Gamma_D$ operator can be employed to characterize admissible and also complete labellings:

\begin{restatable}{prop}{modelcomplete}\label{p:modelcomplete}
Let $D = (S, L, C^\varphi)$ be an $\adf$. We have

\begin{itemize}
    \item A labelling $v$ over $S$ is an admissible labelling of $D$ iff $v \leq_i \Gamma_D(v)$.
    \item A labelling $v$ over $S$ is a complete labelling of $D$ iff $v = \Gamma_D(v)$.
\end{itemize}
\end{restatable}

In addition, we define an labelling $v$ over $S$ is a model of $D$ iff $\Gamma_D(v) \leq_i v$. It is worthy noting our definition of model is different from that introduced in \cite{brewka2010abstract}. While there models and admissible labellings coincide with each other, in the present work, models in general are not admissible. Indeed, we associate admissible labellings with the post-fixpoints of $\Gamma_D$ operator, whereas models are associated with the pre-fixpoints of $\Gamma_D$ operator. We emphasize anyway our defense of this characterization of models is freely inspired by how models are usually defined in logic programming (see \cite{przymusinski90well-founded} for more details).

An important notion introduced in this work is exhibited in the sequel; it is an adaptation to $\adf$s of the well-known concept of \emph{reduct} found in logic programming \cite{gelfond1988stable}:

\begin{mdef}\label{d:reduct} 
Let $D = (S, L, C^\tr)$ be an $\adf$, and $v$ a labelling over $S$. The reduct $D_v = (S, L, C^\tr_v))$ is an $\adf$ such that for every $s \in S$, $C^\tr_{v_s} = C^\tr_s$ if there exists $\set{a_1, \ldots, a_m, \neg b_1, \ldots, \neg b_n} \in C^\tr_s$ such that $v(a_1 \wedge \cdots \wedge a_m \wedge \neg b_1 \wedge \cdots \wedge \neg b_n) \neq \fa$; otherwise,  $C^\tr_{v_s} = \emptyset$. Alternatively, the reduct can be defined as $D_v = (S, L, C^\varphi_v))$, where for every $s \in S$, we have ${\varphi_v}_s = \varphi_s$ if ${C^\tr_v}_s = C^\tr_s$; otherwise, ${\varphi_v}_s = \fa$.
\end{mdef}

When introducing some semantics for $\adf$s, we will resort to the set of undefined statements of a labelling $v$ over $S$, denoted by $\undec(v) = \set{s \in S \mid v(s) = \un}$. Now some of the main semantics for an $\adf$ can be defined as follows:

\begin{mdef}\label{d:semantics}
Let $D = (S, L, C^\varphi)$ be an $\adf$, and $v$ a labelling over $S$. We have

\begin{itemize}
    \item $v$ is a grounded model of $D$ iff $v$ is the $\leq_i$-least complete model of $D$.
    \item $v$ is a partial stable model of $D$ iff $v$ is the $\leq_i$-least complete model of $D_v$.
    \item $v$ is a preferred model of $D$ iff $v$ is a $\leq_i$-maximal admissible labelling of $D$.
    \item $v$ is a regular model of $D$ iff $v$ is $\leq_i$-maximal partial stable model of $D$.
    \item $v$ is a stable model of $D$ iff $v$ is a two-valued partial stable model of $D$.
    \item $v$ is a semi-stable model of $D$ iff $v$ is a complete model of $D$ with minimal (wrt set inclusion) $\undec(v)$.
    \item $v$ is an L-stable model of $D$ iff $v$ is a partial stable model of $D$ with minimal (wrt set inclusion) $\undec(v)$.
\end{itemize}
\end{mdef}

From Definition \ref{d:complete}, it follows the grounded model is unique for each $\adf$ $D$ and corresponds to the least fixpoint of $\Gamma_D$ operator. 

\begin{example}\label{ex:adf}
Consider the $\adf$ $D = (S, C^\varphi)$ given by
\[ a [\top] \qquad b[\neg a \vee c] \qquad c [b] \]
where $S= \set{a, b, c}$, and the acceptance formula of each statement $s \in S$ is written in square brackets on the right of $s$.
It has as semantics

\begin{itemize}
    \item $\set{a, b, c}$, $\set{a, \neg b, \neg c}$ and $\set{a}$ are the complete models of $D$.
    \item $\set{a}$ is the grounded model of $D$.
    \item $\set{a, \neg b, \neg c}$ and $\set{a}$ are the partial models of $D$.
    \item $\set{a, b, c}$ and $\set{a, \neg b, \neg c}$ are the preferred models of $D$.
    \item $\set{a, \neg b, \neg c}$ is the unique regular model of $D$.
    \item $\set{a, \neg b, \neg c}$ is the unique stable model of $D$
    \item $\set{a, b, c}$ and $\set{a, \neg b, \neg c}$ are semi-stable models of $D$. 
    \item $\set{a, \neg b, \neg c}$ is the unique L-stable model of $D$.
\end{itemize}
\end{example}

Furthermore, every partial stable model of an $\adf$ $D$ is a complete model of $D$:

\begin{restatable}{lmm}{completedv}\label{l:completedv}
Let $D$ be an $\adf$. We have $v$ is a complete model of $D_v$ iff $v$ is a complete model of $D$.
\end{restatable}

\begin{restatable}{theo}{partial}\label{t:partial}
Let $D$ be an $\adf$. If $v$ is a partial stable model of $D$, then $v$ is a complete model of $D$.
\end{restatable}

The converse result is not guaranteed to hold, i.e., not all complete model of $D$ is a partial stable model of $D$:

\begin{example}
Recalling $\adf$ of Example \ref{ex:adf}, we see $\set{a,b,c}$ is a complete model of $D$, but it is not a partial model of $D$.
\end{example}

The following results involving grounded models can also be obtained:

\begin{restatable}{theo}{grounded}\label{t:grounded}
For any $\adf$ $D = (S, L, C^\varphi)$, the following statements are equivalent:

\begin{enumerate}[a)]
    \item $v$ is a grounded model of $D$.
    \item $v$ is the $\leq_i$-least partial model of $D$.
    \item $v$ is the $\leq_i$-least model of $D$.
\end{enumerate}
\end{restatable}

We also identify the relations below involving the semantics we have defined:

\begin{restatable}{theo}{general}\label{t:general}
Let $D$ be an $\adf$.

\begin{itemize}
    %\item Each preferred model of $D$ is a complete model of $D$, but not vice versa.
    \item $v$ is a preferred model of $D$ iff $v$ is $\leq_i$-maximal complete model of $D$.
   % \item If $v$ is a regular model of $D$, then $v$ is a preferred model of $D$, but not vice versa.
    \item If $D$ has at least one stable model, then $v$ is a stable model of $D$ iff $v$ is an L-stable model of $D$.
    \item If $v$ is a stable model of $D$, then $v$ is a semi-stable model of $D$, but not vice versa.
    %\item If $v$ is an L-stable model of $D$, then $v$ is a semi-stable model of $D$, but not vice versa.
\end{itemize}
\end{restatable}

On the other hand, we identify the following negative results:

\begin{restatable}{prop}{negative}\label{p:negative}
Let $D$ be an $\adf$.

\begin{itemize}
    \item Not all preferred model of $D$ is a regular model of $D$.
    \item Not all regular model of $D$ is a preferred model of $D$.
    \item Not all L-stable model of $D$ is a semi-stable model of $D$.
    \item Not all semi-stable model of $D$ is an $L$-stable model of $D$.
\end{itemize}
\end{restatable}

From these results it is clear each preferred model of $D$ is a complete model of $D$, but not vice versa. Furthermore,
they also show those semantics based on partial models are not a particular case of the corresponding semantics based on complete models. However, in the next section we will show when we restrain our attention to the subclass of $\adf$s corresponding to $\af$s, these semantics coincide with each other.
